TACTiS-2: Better, Faster, Simpler Attentional Copulas for Multivariate Time Series

We introduce a new model for multivariate probabilistic time series prediction, designed to flexibly address a range of tasks including forecasting, interpolation, and their combinations. Building on copula theory, we propose a simplified objective for the recently-introduced transformer-based attentional copulas (TACTiS), wherein the number of distributional parameters now scales linearly with the number of variables instead of factorially. The new objective requires the introduction of a training curriculum, which goes hand-in-hand with necessary changes to the original architecture. We show that the resulting model has significantly better training dynamics and achieves state-of-the-art performance across diverse real-world forecasting tasks, while maintaining the flexibility of prior work, such as seamless handling of unaligned and unevenly-sampled time series. Code is made available at https://github.com/ServiceNow/TACTiS.

==> backup_att_copula.tex <==
One solution to this challenge has been proposed by \citet{tactis}, who showed that non-parametric copulas can be learned by combining normalizing flows and attention mechanisms with a permutation-based objective.
Their approach is as follows.
First, they model each marginal $\{F_{\phi_i}\}_{i=1}^n$ with a \emph{Deep Sigmoidal Flow}~\citep{huang18-naf} to ensure that they are well-defined, i.e., continuous, monotonically increasing, and mapping to the unit interval $[0, 1]$.
Second, they consider a factorization of the copula density $c_{\phi_c}$ based on the chain rule of probability according to an arbitrary permutation of the variables $\pi = [\pi_1, \ldots, \pi_{n}] \in \Pi$, where $\Pi$ is the set of all $n!$ permutations of $[1, \ldots, n]$. The resulting copula density, $c_{\phi_{c}^{\pi}}$, can be written as:
\begin{equation}
    \label{eq:copula-density}
    c_{\phi_{c}^{\pi}}\!\left(u_1, \ldots, u_{n} \right) \eqdef c_{\phi_{c1}^{\pi}}\!\!\left(u_{\pi_1}\right) \times c_{\phi_{c2}^{\pi}}\!\!\left(u_{\pi_2} \mid u_{\pi_1}\right) \times \cdots \times
    c_{\phi^{\pi}_{c{n}}}\!\!\left(u_{\pi_{n}} \mid u_{\pi_1}, \ldots, u_{\pi_{n - 1}} \right),
\end{equation}
where $u_{\pi_k} = F_{\phi_{\pi_k}}\!\big(x_{\pi_k}\big)$ and the $c_{\phi_{ci}^{\pi}}$ are arbitrary distributions (e.g., histograms) on the unit interval whose parameters $\phi_{ci}^{\pi}$ are produced by an attention mechanism.
There is, however, one important exception: the density of the first variable in the permutation $c_{\phi_{c1}^{\pi}}$ is always taken to be the \emph{density of a uniform distribution} $\uniform{0}{1}$ and thus $c_{\phi_{c1}^{\pi}}\!\!\left(u_{\pi_1}\right) = 1$.
% This choice is motivated by the fact that any copula must have uniform marginals and that the first term in the chain rule of probability is a marginal density.
This choice, combined with solving the following permutation-based problem, guarantees that, at the minimum, all of the $c_{\phi_{c}^{\pi}}$, irrespective of $\pi$, are equivalent and correspond to the density of a valid copula:
\begin{equation}\label{eq:copula-based-density-estimator}
    \argmin_{\phi_1, \ldots, \phi_n, \phib_c^{\Pi}} \;\; \expect_{\Xb \sim \Scal} \expect_{\pi \sim \Pi} -\log c_{\phi_{c}^{\pi}}\Big( 
        F_{\phi_{1}}\!\big(x_{1}\big), F_{\phi_{2}}\!\big(x_{2}\big), \ldots, F_{\phi_{n}}\!\big(x_{n}\big)
    \!\Big)  \;\times
    f_{\phi_1}\!\big(x_1\big) \times \cdots \times f_{\phi_{n}}\!\big(x_{n}\big),
\end{equation}
where $\phib_c^\Pi \eqdef \{ \phi_{c1}^{\pi}, \ldots \phi_{cn}^{\pi} \}_{\pi \in \Pi}$ are the parameters for each of the $n!$ factorizations of the copula density (see \citet{tactis}, Theorem 1).
